qRobot: A Quantum computing approach in mobile robot order picking and batching problem solver optimization

This article aims to bring quantum computing to robotics. A quantum algorithm is developed to minimize the distance travelled in warehouses and distribution centres where order picking is applied. For this, a proof of concept is proposed through a Raspberry Pi 4, generating a quantum combinatorial optimization algorithm that saves the distance travelled and the batch of orders to be made. In case of computational need, the robot will be able to parallelize part of the operations in hybrid computing (quantum + classical), accessing CPUs and QPUs distributed in a public or private cloud. Before this, we must develop a stable environment (ARM64) inside the robot (Raspberry) to run gradient operations and other quantum algorithms on IBMQ, Amazon Braket, D'wave and Pennylane locally or remotely. The proof of concept will run in such quantum environments above.

==> images/back.tex <==
\begin{table}[t!]
    \centering
    \begin{tabular}{c|c|c}
      \hline
        Initial\_point  &  Schedule  &  Solution Class \\
         \hline
         &   &   &
          \hline
    \end{tabular}
    \caption{(a) qCBR's Memory structure - Solution class}
    \label{tab:(a)sol_class}
    \begin{tabular}{c|c}
      \hline
        solution class   &   Schedule \\
         \hline
         &   &   
          \hline
    \end{tabular}
    \caption{(b) qCBR's Memory structure - Training data}
    \label{tab:(b)train_data}
    \begin{tabular}{c|c}
      \hline
        solution class   &   Schedule \\
        \hline
        &   &   
        \hline
        &   &
        \hline
        &   & 
        \hline
        Cross-validation - (Leave One Out) & -- \\
        \hline
        &   &
        \hline
        &   &   
        \hline
        &   &   
        \hline
    \end{tabular}
    \caption{(c) qCBR's Memory structure. The use the cross-validation technique helps to improve the quality of the classifier training\cite{Mic}. - Test data}
    \label{tab:(c)test_data}
\end{table}


\begin{table}[t!]
    \centering
    \begin{tabular}{c|c|c|c}
        solution class &  Initial\_point\_{1}  & ... &  Initial\_point\_{N} \\
         \hline
        A  &  ...   & ...   & ...  \\
         \hline
    \end{tabular}
    \caption{Memory structure used for the Training System. A label identifies each class. And in this case, A is one of the labels. For more detail, refer to the code \cite{Ade21}.}
    \label{tab:mem_struture}
\end{table}
